Complete element abundances of nine stars in the r-process galaxy Reticulum II

We present chemical abundances derived from high-resolution Magellan/MIKE spectra of the nine brightest known red giant members of the ultra-faint dwarf galaxy Reticulum II. These stars span the full metallicity range of Ret II (-3.5 < [Fe/H] < -2). Seven of the nine stars have extremely high levels of r-process material ([Eu/Fe]~1.7), in contrast to the extremely low neutron-capture element abundances found in every other ultra-faint dwarf galaxy studied to date. The other two stars are the most metal-poor stars in the system ([Fe/H] < -3), and they have neutron-capture element abundance limits similar to those in other ultra-faint dwarf galaxies. We confirm that the relative abundances of Sr, Y, and Zr in these stars are similar to those found in r-process halo stars but ~0.5 dex lower than the solar r-process pattern. If the universal r-process pattern extends to those elements, the stars in Ret II display the least contaminated known r-process pattern. The abundances of lighter elements up to the iron peak are otherwise similar to abundances of stars in the halo and in other ultra-faint dwarf galaxies. However, the scatter in abundance ratios is large enough to suggest that inhomogeneous metal mixing is required to explain the chemical evolution of this galaxy. The presence of low amounts of neutron-capture elements in other ultra-faint dwarf galaxies may imply the existence of additional r-process sites besides the source of r-process elements in Ret II. Galaxies like Ret II may be the original birth sites of r-process enhanced stars now found in the halo.

==> ew_final.tex <==
\begin{deluxetable*}{llrrrrrrrrrrrrrrrrrrrr}
\tablecolumns{22}
\tablewidth{0pt}
\tabletypesize{\footnotesize}
\tabletypesize{\tiny}
\tablecaption{Equivalent Widths\label{tbl:ew}}
\tablehead{\colhead{El.} & \colhead{$\lambda$} & \colhead{$\chi$} & \colhead{$\log gf$} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon(X)$ (dex)} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon(X)$ (dex)} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon(X)$ (dex)} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon(X)$ (dex)} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon(X)$ (dex)} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon(X)$ (dex)} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon(X)$ (dex)} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon(X)$ (dex)} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon(X)$ (dex)}\\
\colhead{} & \colhead{(\AA)} & \colhead{(eV)} & \colhead{(dex)} & \multicolumn{2}{c}{\RetA} & \multicolumn{2}{c}{\RetB} & \multicolumn{2}{c}{\RetC} & \multicolumn{2}{c}{\RetD} & \multicolumn{2}{c}{\RetE} & \multicolumn{2}{c}{\RetF} & \multicolumn{2}{c}{\RetG} & \multicolumn{2}{c}{\RetH} & \multicolumn{2}{c}{\RetI}}
\startdata
CH    &  4313    &\nodata&  \nodata &     syn &    6.07 &     syn &    5.86 &     syn &    5.67 &     syn &    5.24 &     syn &    6.74 &     syn &    6.00 &     syn & $< 6.09$&     syn &    6.70 &     syn &    6.51 \\
CH    &  4323    &\nodata&  \nodata &     syn &    6.07 &     syn &    5.86 &     syn &    5.77 &     syn &    5.34 &     syn &    6.74 &     syn &    5.70 &     syn & $< 6.09$&     syn &    6.70 &     syn &    6.51 \\
Na I  &  5889.95 &  0.00 & $  0.11$ &   178.6 &    3.59 &   152.0 &    3.51 &   146.0 &    3.56 &   179.4 &    3.88 &   156.9 &    3.97 &   114.3 &    3.40 &   104.1 &    3.21 &   148.9 &    4.04 &   112.0 &    3.53 \\
Na I  &  5895.92 &  0.00 & $ -0.19$ &   151.9 &    3.47 &   124.2 &    3.33 &   142.8 &    3.80 &   154.2 &    3.86 &   136.2 &    3.96 &   125.1 &    3.90 &    83.2 &    3.15 &   159.8 &    4.47 &    76.1 &    3.20 \\
Mg I  &  3829.36 &  2.71 & $ -0.21$ & \nodata & \nodata & \nodata & \nodata &   164.7 &    5.08 &   146.5 &    4.84 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mg I  &  3986.75 &  4.35 & $ -1.03$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    54.0 &    5.97 & \nodata & \nodata \\
Mg I  &  4167.27 &  4.35 & $ -0.71$ &    57.7 &    5.24 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    85.3 &    6.07 & \nodata & \nodata \\
Mg I  &  4571.10 &  0.00 & $ -5.69$ &    76.3 &    5.17 & \nodata & \nodata &    54.6 &    5.34 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    39.8 &    5.72 & \nodata & \nodata \\
Mg I  &  4702.99 &  4.33 & $ -0.38$ &    49.5 &    4.73 & \nodata & \nodata & \nodata & \nodata &    47.1 &    4.86 &    59.4 &    5.16 &    62.8 &    5.24 & \nodata & \nodata &    82.4 &    5.54 & \nodata & \nodata \\
Mg I  &  5172.68 &  2.71 & $ -0.45$ & \nodata & \nodata &   175.4 &    5.00 &   147.8 &    4.74 &   164.0 &    4.98 &   217.9 &    5.59 &   138.8 &    4.88 &   111.5 &    4.41 &   193.7 &    5.47 &   138.9 &    4.93 \\
Mg I  &  5183.60 &  2.72 & $ -0.24$ & \nodata & \nodata &   187.1 &    4.94 &   235.6 &    5.39 &   199.7 &    5.12 &   197.3 &    5.24 &   137.3 &    4.66 &   156.7 &    4.78 & \nodata & \nodata &   177.8 &    5.08 \\
Mg I  &  5528.40 &  4.34 & $ -0.50$ &    65.4 &    5.05 &    59.3 &    5.09 & \nodata & \nodata &    46.1 &    4.96 & \nodata & \nodata &    65.0 &    5.42 & \nodata & \nodata &    84.8 &    5.80 & \nodata & \nodata \\
Al I  &  3961.52 &  0.01 & $ -0.34$ &   139.9 &    2.93 &   116.2 &    2.74 &   110.4 &    2.79 &    78.7 &    2.16 & $<145.5$& $< 3.66$& $<135.2$& $< 3.60$& $< 88.4$& $< 2.71$&   124.0 &    3.53 & $<142.7$& $< 3.76$\\
Al I  &  3944    &  0.00 & $ -0.62$ &    syn  &    2.63 & \nodata & \nodata & \nodata & \nodata &     syn &    2.71 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &     syn &    3.23 & \nodata & \nodata \\
Si I  &  3905.52 &  1.91 & $ -1.09$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &     syn &    4.37 & \nodata & \nodata &     syn &    5.08 & \nodata & \nodata &     syn &    5.98 & \nodata & \nodata \\
Si I  &  4102.94 &  1.91 & $ -3.14$ &    91.5 &    5.19 &    61.9 &    4.99 &    46.6 &    4.86 &    56.4 &    5.05 &    60.2 &    5.34 & \nodata & \nodata & $< 59.3$& $< 5.49$&    79.6 &    5.98 & $<158.0$& $< 7.27$\\
Ca I  &  4226.73 &  0.00 & $  0.24$ & \nodata & \nodata & \nodata & \nodata &   185.6 &    3.69 &   145.5 &    3.25 & \nodata & \nodata &   165.8 &    3.74 &   108.4 &    2.87 & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  4283.01 &  1.89 & $ -0.22$ & \nodata & \nodata &    63.8 &    3.98 &    60.5 &    4.03 &    28.3 &    3.45 &    76.3 &    4.53 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  4318.65 &  1.89 & $ -0.21$ &    39.7 &    3.41 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    68.1 &    4.35 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  4425.44 &  1.88 & $ -0.36$ & \nodata & \nodata &    37.5 &    3.66 & \nodata & \nodata & \nodata & \nodata &    57.2 &    4.25 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  4434.96 &  1.89 & $ -0.01$ &    57.4 &    3.48 & \nodata & \nodata &    53.5 &    3.67 &    27.2 &    3.20 &    93.7 &    4.63 &    37.4 &    3.60 & \nodata & \nodata &    91.3 &    4.76 &    46.0 &    3.93 \\
Ca I  &  4435.69 &  1.89 & $ -0.52$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    70.1 &    4.67 &    36.8 &    4.10 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  4454.78 &  1.90 & $  0.26$ &    67.0 &    3.37 &    83.8 &    3.84 &    63.7 &    3.59 &    35.0 &    3.10 &    86.6 &    4.22 &    59.9 &    3.77 & \nodata & \nodata & \nodata & \nodata &    62.9 &    3.99 \\
Ca I  &  4455.89 &  1.90 & $ -0.53$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    53.8 &    4.56 & \nodata & \nodata \\
Ca I  &  5265.56 &  2.52 & $ -0.26$ & \nodata & \nodata &    23.6 &    3.98 & \nodata & \nodata & \nodata & \nodata &    47.7 &    4.65 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  5588.76 &  2.52 & $  0.21$ &    34.3 &    3.58 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    86.5 &    4.92 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  5594.47 &  2.52 & $  0.10$ &    28.6 &    3.58 &    27.3 &    3.69 & \nodata & \nodata & \nodata & \nodata &    48.0 &    4.29 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  6102.72 &  1.88 & $ -0.79$ &    26.6 &    3.64 &    22.6 &    3.71 & \nodata & \nodata & \nodata & \nodata &    51.6 &    4.51 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  6122.22 &  1.89 & $ -0.32$ &    49.8 &    3.57 &    27.5 &    3.37 & \nodata & \nodata &    38.8 &    3.66 &    71.0 &    4.39 & \nodata & \nodata &    16.7 &    3.42 &    77.5 &    4.69 & \nodata & \nodata \\
Ca I  &  6162.17 &  1.90 & $ -0.09$ &    67.1 &    3.59 &    47.5 &    3.50 & \nodata & \nodata &    28.7 &    3.25 &   113.5 &    4.92 & \nodata & \nodata & \nodata & \nodata &    72.0 &    4.37 &    52.5 &    4.05 \\
Ca I  &  6169.06 &  2.52 & $ -0.80$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    29.2 &    4.81 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  6439.07 &  2.52 & $  0.47$ &    51.5 &    3.56 &    66.9 &    3.95 & \nodata & \nodata & \nodata & \nodata &    77.3 &    4.44 & \nodata & \nodata &    20.1 &    3.39 &    71.2 &    4.51 & \nodata & \nodata \\
Sc II &  4246.82 &  0.32 & $  0.24$ &     syn &   -0.16 &     syn &    0.53 &     syn &    0.34 &     syn &   -0.09 &     syn &    0.25 &     syn &    0.12 &     syn &   -0.29 &     syn &    1.32 &     syn &    0.54 \\
Sc II &  4314.08 &  0.62 & $ -0.10$ &     syn &   -0.11 &     syn &    0.53 &     syn &    0.04 &     syn &    0.21 &     syn &    0.36 &     syn &    0.32 & \nodata & \nodata &     syn &    1.67 & \nodata & \nodata \\
Sc II &  4325.00 &  0.59 & $ -0.44$ &     syn &   -0.06 &     syn &    0.18 &     syn &   -0.01 &     syn &    0.01 &     syn &    0.06 &     syn &    0.62 & \nodata & \nodata &     syn &    1.17 & \nodata & \nodata \\
Sc II &  4400.39 &  0.61 & $ -0.54$ &     syn &    0.04 &     syn &    0.18 &     syn &    0.04 &     syn &    0.21 &     syn &    0.46 &     syn &    0.62 & \nodata & \nodata &     syn &    1.42 & \nodata & \nodata \\
Sc II &  4415.54 &  0.59 & $ -0.67$ &     syn &    0.14 &     syn &    0.18 &     syn &    0.37 &     syn &    0.21 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &     syn &    1.27 & \nodata & \nodata \\
Ti I  &  3989.76 &  0.02 & $ -0.06$ &    89.0 &    2.37 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    88.1 &    3.29 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  3998.64 &  0.05 & $  0.01$ &    63.8 &    1.88 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4008.93 &  0.02 & $ -1.02$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    35.8 &    3.12 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4533.25 &  0.85 & $  0.53$ &    46.7 &    2.02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    68.0 &    3.05 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4534.78 &  0.84 & $  0.34$ &    29.2 &    1.90 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    72.6 &    3.32 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4535.57 &  0.83 & $  0.12$ &    25.1 &    2.02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    45.3 &    3.00 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4656.47 &  0.00 & $ -1.29$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    37.3 &    3.33 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4681.91 &  0.05 & $ -1.01$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    37.3 &    3.10 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4981.73 &  0.84 & $  0.56$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    63.3 &    2.87 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4999.50 &  0.83 & $  0.31$ &    54.2 &    2.29 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  5192.97 &  0.02 & $ -0.95$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    57.8 &    3.34 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  5210.39 &  0.05 & $ -0.83$ &    37.9 &    2.20 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    52.0 &    3.15 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  3913.46 &  1.12 & $ -0.42$ & \nodata & \nodata & \nodata & \nodata &    89.6 &    1.96 &    80.6 &    1.87 &   139.5 &    3.59 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4025.12 &  0.61 & $ -1.98$ &    70.2 &    1.94 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    82.6 &    3.19 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4028.34 &  1.89 & $ -0.96$ &    82.7 &    2.72 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    84.6 &    3.66 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4053.83 &  1.89 & $ -1.21$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    55.4 &    3.25 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4161.53 &  1.08 & $ -2.16$ & \nodata & \nodata &    28.1 &    2.27 & \nodata & \nodata & \nodata & \nodata &    72.9 &    3.64 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4163.63 &  2.59 & $ -0.40$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    79.4 &    3.72 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4184.31 &  1.08 & $ -2.51$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    52.7 &    3.58 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4290.22 &  1.16 & $ -0.93$ & \nodata & \nodata &    90.7 &    2.22 &    93.4 &    2.48 &    59.6 &    1.88 &   119.0 &    3.59 &    61.2 &    2.30 & \nodata & \nodata &    79.3 &    3.00 & \nodata & \nodata \\
Ti II &  4300.05 &  1.18 & $ -0.49$ & \nodata & \nodata & \nodata & \nodata &    89.5 &    1.99 &    73.4 &    1.74 & \nodata & \nodata &    98.9 &    2.85 & \nodata & \nodata &   117.9 &    3.53 &    71.0 &    2.52 \\
Ti II &  4330.72 &  1.18 & $ -2.06$ &    61.6 &    2.55 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    64.8 &    3.45 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4337.91 &  1.08 & $ -0.96$ &   127.8 &    2.55 &   104.3 &    2.43 &    95.8 &    2.46 &    80.7 &    2.25 &   109.1 &    3.28 &    82.6 &    2.76 &    51.1 &    2.21 &    90.5 &    3.23 &    76.9 &    3.04 \\
Ti II &  4394.06 &  1.22 & $ -1.78$ &    55.6 &    2.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    81.5 &    3.57 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4395.03 &  1.08 & $ -0.54$ & \nodata & \nodata &   111.1 &    2.15 &    98.4 &    2.10 &    90.9 &    2.07 &   121.1 &    3.12 &    99.3 &    2.77 &    41.1 &    1.60 &   102.9 &    3.11 & \nodata & \nodata \\
Ti II &  4395.84 &  1.24 & $ -1.93$ &    46.8 &    2.26 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4399.77 &  1.24 & $ -1.19$ &    76.3 &    1.97 &    73.5 &    2.22 &    68.9 &    2.30 &    59.7 &    2.22 &   110.6 &    3.71 &    68.2 &    2.80 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4417.71 &  1.17 & $ -1.19$ &    98.2 &    2.27 &    78.5 &    2.23 &    64.4 &    2.13 &    64.2 &    2.22 &    87.0 &    3.04 & \nodata & \nodata & \nodata & \nodata &    80.2 &    3.27 &    60.2 &    2.92 \\
Ti II &  4418.33 &  1.24 & $ -1.97$ &    44.3 &    2.26 &    59.6 &    2.78 & \nodata & \nodata & \nodata & \nodata &    54.1 &    3.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4441.73 &  1.18 & $ -2.41$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    46.2 &    3.45 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4443.80 &  1.08 & $ -0.72$ &   111.1 &    1.92 &   114.1 &    2.38 &    99.9 &    2.30 &    76.5 &    1.89 &   116.7 &    3.19 &    76.2 &    2.33 & \nodata & \nodata &    94.1 &    3.05 &    61.6 &    2.38 \\
Ti II &  4444.55 &  1.12 & $ -2.24$ &    47.2 &    2.42 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    69.6 &    3.65 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4450.48 &  1.08 & $ -1.52$ &    67.4 &    1.95 &    74.4 &    2.37 &    70.5 &    2.46 &    47.6 &    2.14 &    83.7 &    3.19 & \nodata & \nodata & \nodata & \nodata &    64.4 &    3.11 & \nodata & \nodata \\
Ti II &  4464.45 &  1.16 & $ -1.81$ &    55.4 &    2.16 &    46.1 &    2.30 &    48.4 &    2.46 & \nodata & \nodata &    85.6 &    3.61 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4468.52 &  1.13 & $ -0.60$ &   137.4 &    2.40 &   129.2 &    2.65 &    96.4 &    2.14 &    90.5 &    2.15 &   124.8 &    3.29 &    71.0 &    2.13 & \nodata & \nodata &   109.0 &    3.35 &    56.8 &    2.20 \\
Ti II &  4470.85 &  1.17 & $ -2.02$ &    32.4 &    2.02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    68.7 &    3.47 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4501.27 &  1.12 & $ -0.77$ &   117.9 &    2.15 &   102.3 &    2.20 &    83.8 &    2.02 &    78.7 &    2.03 &   125.3 &    3.45 &    89.1 &    2.75 &    66.0 &    2.34 &   107.8 &    3.47 &    67.3 &    2.61 \\
Ti II &  4529.48 &  1.57 & $ -2.03$ &    22.2 &    2.30 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    46.3 &    3.50 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4533.96 &  1.24 & $ -0.53$ &   122.7 &    2.15 & \nodata & \nodata &    88.2 &    2.00 &    70.0 &    1.74 &   113.1 &    3.07 &    68.2 &    2.12 &    40.6 &    1.74 &   121.0 &    3.64 &    85.5 &    2.97 \\
Ti II &  4563.77 &  1.22 & $ -0.96$ &   109.7 &    2.28 &    86.9 &    2.18 &    72.9 &    2.10 &    74.3 &    2.23 &   105.7 &    3.29 &    76.7 &    2.72 &    50.8 &    2.33 &   102.5 &    3.63 &    61.4 &    2.75 \\
Ti II &  4571.97 &  1.57 & $ -0.32$ &   106.6 &    2.01 &    92.6 &    2.08 &    91.5 &    2.24 &    69.8 &    1.91 &   124.4 &    3.47 &    56.7 &    2.02 &    44.5 &    1.96 &   107.3 &    3.48 &    52.1 &    2.28 \\
Ti II &  4589.91 &  1.24 & $ -1.79$ &    60.8 &    2.30 &    57.6 &    2.54 & \nodata & \nodata & \nodata & \nodata &    66.3 &    3.25 & \nodata & \nodata & \nodata & \nodata &    61.5 &    3.48 & \nodata & \nodata \\
Ti II &  4657.20 &  1.24 & $ -2.24$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    37.3 &    3.16 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4708.66 &  1.24 & $ -2.34$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    49.7 &    3.48 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4779.98 &  2.05 & $ -1.37$ &    24.8 &    2.26 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    43.0 &    3.29 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4798.53 &  1.08 & $ -2.68$ &    29.7 &    2.49 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    41.7 &    3.50 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4805.09 &  2.06 & $ -1.10$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    57.0 &    3.29 & \nodata & \nodata & \nodata & \nodata &    56.2 &    3.54 & \nodata & \nodata \\
Ti II &  5129.16 &  1.89 & $ -1.24$ &    34.6 &    2.10 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  5188.69 &  1.58 & $ -1.05$ &    73.2 &    2.10 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    85.0 &    3.22 &    48.2 &    2.55 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  5226.54 &  1.57 & $ -1.26$ &    66.1 &    2.19 &    66.1 &    2.47 & \nodata & \nodata & \nodata & \nodata &    78.0 &    3.26 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  5336.79 &  1.58 & $ -1.59$ &    50.1 &    2.30 & \nodata & \nodata & \nodata & \nodata &    22.2 &    2.22 &    71.5 &    3.47 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  4254.33 &  0.00 & $ -0.11$ &   109.0 &    1.94 &   102.4 &    2.21 &   106.6 &    2.56 &    85.1 &    2.11 &   129.2 &    3.39 &    84.4 &    2.55 &    31.1 &    1.43 &   105.2 &    3.26 & \nodata & \nodata \\
Cr I  &  4274.80 &  0.00 & $ -0.22$ &   114.8 &    2.18 &   102.4 &    2.31 &    82.3 &    2.07 &    77.3 &    2.02 &   124.8 &    3.41 & \nodata & \nodata &    40.8 &    1.74 &   109.6 &    3.46 & \nodata & \nodata \\
Cr I  &  4289.72 &  0.00 & $ -0.37$ & \nodata & \nodata &   105.8 &    2.54 & \nodata & \nodata &    73.2 &    2.08 &   117.9 &    3.42 &    72.2 &    2.47 & \nodata & \nodata & \nodata & \nodata &    54.2 &    2.37 \\
Cr I  &  4337.57 &  0.97 & $ -1.11$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    46.1 &    3.61 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  4616.14 &  0.98 & $ -1.19$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    42.9 &    3.62 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  4626.19 &  0.97 & $ -1.32$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    35.9 &    3.60 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  4646.15 &  1.03 & $ -0.74$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    48.4 &    3.33 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  4652.16 &  1.00 & $ -1.03$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    42.8 &    3.48 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  5206.04 &  0.94 & $  0.02$ &    70.7 &    2.12 &    70.8 &    2.41 & \nodata & \nodata & \nodata & \nodata &    95.6 &    3.39 & \nodata & \nodata & \nodata & \nodata &    80.6 &    3.38 & \nodata & \nodata \\
Cr I  &  5208.42 &  0.94 & $  0.16$ & \nodata & \nodata &    94.7 &    2.71 &    98.8 &    2.98 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  5345.80 &  1.00 & $ -0.95$ &    32.4 &    2.57 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  5409.77 &  1.03 & $ -0.67$ &    29.3 &    2.27 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    62.9 &    3.47 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mn I  &  4030.75 &  0.00 & $ -0.48$ &     syn &    2.02 &     syn &    1.46 &     syn &    1.52 &     syn &    1.54 &     syn &    2.34 &     syn & $< 3.70$&     syn & $< 2.69$&     syn &    2.85 &     syn & $< 4.17$\\
Mn I  &  4033.06 &  0.00 & $ -0.62$ &     syn &    1.92 &     syn &    1.66 &     syn &    1.32 &     syn &    1.09 &     syn &    2.64 & \nodata & \nodata & \nodata & \nodata &     syn &    2.45 & \nodata & \nodata \\
Mn I  &  4034.48 &  0.00 & $ -0.81$ &     syn &    1.92 &     syn &    1.66 &     syn &    1.72 &     syn &    1.39 &     syn &    2.84 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mn I  &  4041.36 &  2.11 & $  0.28$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &     syn &    3.13 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mn I  &  4754.05 &  2.28 & $ -0.09$ &     syn &    2.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &     syn &    3.04 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mn I  &  4823.53 &  2.32 & $  0.14$ &     syn &    2.12 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &     syn &    3.04 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3743.36 &  0.99 & $ -0.79$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   105.4 &    4.18 & \nodata & \nodata & \nodata & \nodata &    69.8 &    3.67 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3753.61 &  2.18 & $ -0.89$ & \nodata & \nodata &    82.8 &    4.72 & \nodata & \nodata & \nodata & \nodata &    82.7 &    5.23 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3758.23 &  0.96 & $ -0.01$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   103.7 &    3.73 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3765.54 &  3.24 & $  0.48$ &    84.6 &    4.36 &    67.0 &    4.23 & \nodata & \nodata & \nodata & \nodata &    89.4 &    5.15 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3767.19 &  1.01 & $ -0.39$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   106.0 &    4.20 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3786.68 &  1.01 & $ -2.19$ & \nodata & \nodata & \nodata & \nodata &    75.2 &    4.66 &    54.7 &    4.26 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3787.88 &  1.01 & $ -0.84$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   101.7 &    4.13 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3805.34 &  3.30 & $  0.31$ & \nodata & \nodata & \nodata & \nodata &    74.7 &    4.78 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3815.84 &  1.48 & $  0.24$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   101.0 &    3.92 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3825.88 &  0.91 & $ -0.02$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   122.4 &    4.02 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3827.82 &  1.56 & $  0.09$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   110.6 &    4.02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3840.44 &  0.99 & $ -0.50$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   115.6 &    4.50 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3841.05 &  1.61 & $ -0.04$ & \nodata & \nodata & \nodata & \nodata &   121.0 &    4.35 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3845.17 &  2.42 & $ -1.39$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    51.5 &    5.21 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3849.97 &  1.01 & $ -0.86$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   117.9 &    4.92 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3850.82 &  0.99 & $ -1.75$ & \nodata & \nodata &    98.0 &    4.52 & \nodata & \nodata & \nodata & \nodata &   101.4 &    5.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3852.57 &  2.18 & $ -1.18$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    74.4 &    5.61 & \nodata & \nodata \\
Fe I  &  3856.37 &  0.05 & $ -1.28$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   125.1 &    4.01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3865.52 &  1.01 & $ -0.95$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   100.7 &    4.18 & \nodata & \nodata &   118.6 &    5.02 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3878.02 &  0.96 & $ -0.90$ & \nodata & \nodata & \nodata & \nodata &   119.7 &    4.44 & \nodata & \nodata & \nodata & \nodata &   106.9 &    4.68 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3878.57 &  0.09 & $ -1.38$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    98.5 &    4.02 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3886.28 &  0.05 & $ -1.08$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   115.9 &    4.06 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3887.05 &  0.91 & $ -1.14$ & \nodata & \nodata & \nodata & \nodata &   117.0 &    4.55 &   104.8 &    4.36 & \nodata & \nodata &   104.6 &    4.81 &    79.9 &    4.16 & \nodata & \nodata &    94.4 &    4.86 \\
Fe I  &  3895.66 &  0.11 & $ -1.67$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   117.7 &    4.29 & \nodata & \nodata & \nodata & \nodata &    92.5 &    4.17 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3899.71 &  0.09 & $ -1.51$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   116.4 &    4.07 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    94.8 &    4.40 \\
Fe I  &  3902.95 &  1.56 & $ -0.44$ & \nodata & \nodata & \nodata & \nodata &   116.5 &    4.57 &    89.3 &    3.97 & \nodata & \nodata & \nodata & \nodata &    69.0 &    3.87 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3917.18 &  0.99 & $ -2.15$ &   106.2 &    4.68 &    91.6 &    4.73 &    85.8 &    4.83 &    62.9 &    4.35 &    90.7 &    5.32 & \nodata & \nodata & \nodata & \nodata &    82.4 &    5.50 & \nodata & \nodata \\
Fe I  &  3920.26 &  0.12 & $ -1.73$ & \nodata & \nodata & \nodata & \nodata &   124.2 &    4.39 &   109.8 &    4.16 & \nodata & \nodata &   106.3 &    4.57 &    85.5 &    4.05 & \nodata & \nodata &   111.9 &    4.98 \\
Fe I  &  3922.91 &  0.05 & $ -1.63$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    82.6 &    3.79 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3940.88 &  0.96 & $ -2.60$ &    90.0 &    4.70 &    57.2 &    4.45 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3949.95 &  2.18 & $ -1.25$ & \nodata & \nodata & \nodata & \nodata &    43.7 &    4.40 & \nodata & \nodata &    72.7 &    5.26 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  3977.74 &  2.20 & $ -1.12$ &    65.3 &    4.28 & \nodata & \nodata & \nodata & \nodata &    26.0 &    3.95 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4005.24 &  1.56 & $ -0.58$ & \nodata & \nodata &   119.3 &    4.49 &   126.3 &    4.88 &    89.7 &    4.08 &   123.9 &    5.12 &   100.8 &    4.80 &    56.4 &    3.71 &   105.9 &    5.07 &    87.2 &    4.74 \\
Fe I  &  4007.27 &  2.76 & $ -1.28$ & \nodata & \nodata & \nodata & \nodata &    33.4 &    4.89 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4014.53 &  3.05 & $ -0.59$ &    60.1 &    4.69 & \nodata & \nodata &    41.6 &    4.68 & \nodata & \nodata &    60.5 &    5.27 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4021.87 &  2.76 & $ -0.73$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    70.3 &    5.31 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4032.63 &  1.49 & $ -2.38$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    55.5 &    5.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4045.81 &  1.49 & $  0.28$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   103.7 &    3.89 & \nodata & \nodata &   104.2 &    4.17 \\
Fe I  &  4058.22 &  3.21 & $ -1.11$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    43.4 &    5.60 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4063.59 &  1.56 & $  0.06$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   117.6 &    4.50 &    80.0 &    3.61 & \nodata & \nodata &   109.1 &    4.54 \\
Fe I  &  4067.27 &  2.56 & $ -1.42$ &    48.4 &    4.73 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4071.74 &  1.61 & $ -0.01$ & \nodata & \nodata & \nodata & \nodata &   125.9 &    4.34 &   105.9 &    3.98 & \nodata & \nodata &   111.8 &    4.51 &    83.2 &    3.81 & \nodata & \nodata &   116.7 &    4.77 \\
Fe I  &  4076.63 &  3.21 & $ -0.37$ &    50.1 &    4.49 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4109.80 &  2.85 & $ -0.94$ &    41.7 &    4.49 & \nodata & \nodata &    47.0 &    4.89 & \nodata & \nodata &    47.2 &    5.11 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4132.06 &  1.61 & $ -0.68$ & \nodata & \nodata &   123.6 &    4.70 &   119.7 &    4.85 &    88.5 &    4.17 &   126.7 &    5.29 &    83.8 &    4.48 & \nodata & \nodata &   119.9 &    5.45 & \nodata & \nodata \\
Fe I  &  4132.90 &  2.85 & $ -1.01$ &    34.3 &    4.42 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4134.68 &  2.83 & $ -0.65$ &    50.7 &    4.32 &    29.9 &    4.16 & \nodata & \nodata & \nodata & \nodata &    73.6 &    5.36 & \nodata & \nodata & \nodata & \nodata &    68.9 &    5.54 & \nodata & \nodata \\
Fe I  &  4137.00 &  3.42 & $ -0.45$ &    30.1 &    4.46 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4143.41 &  3.05 & $ -0.20$ &    57.1 &    4.24 &    51.5 &    4.36 &    56.2 &    4.55 &    41.4 &    4.29 &    75.0 &    5.18 & \nodata & \nodata & \nodata & \nodata &    68.2 &    5.29 &    51.1 &    4.97 \\
Fe I  &  4143.87 &  1.56 & $ -0.51$ & \nodata & \nodata &   120.1 &    4.38 &   120.1 &    4.63 &    87.3 &    3.91 &   128.5 &    5.09 &    98.8 &    4.65 &    85.5 &    4.30 & \nodata & \nodata &   102.6 &    4.97 \\
Fe I  &  4147.67 &  1.48 & $ -2.07$ &    70.4 &    4.41 & \nodata & \nodata &    57.4 &    4.63 &    27.8 &    4.09 &    63.7 &    5.05 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4152.17 &  0.96 & $ -3.23$ &    61.9 &    4.79 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    63.2 &    5.62 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4153.90 &  3.40 & $ -0.32$ &    36.0 &    4.42 & \nodata & \nodata &    44.7 &    4.85 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    57.3 &    5.49 & \nodata & \nodata \\
Fe I  &  4154.50 &  2.83 & $ -0.69$ & \nodata & \nodata &    64.3 &    4.81 &    35.0 &    4.39 & \nodata & \nodata &    69.4 &    5.30 & \nodata & \nodata & \nodata & \nodata &    58.4 &    5.31 & \nodata & \nodata \\
Fe I  &  4154.81 &  3.37 & $ -0.40$ & \nodata & \nodata & \nodata & \nodata &    27.5 &    4.56 & \nodata & \nodata &    44.8 &    5.08 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4156.80 &  2.83 & $ -0.81$ &    37.2 &    4.25 &    49.5 &    4.68 &    25.5 &    4.31 & \nodata & \nodata &    61.8 &    5.25 & \nodata & \nodata & \nodata & \nodata &    54.2 &    5.34 & \nodata & \nodata \\
Fe I  &  4157.78 &  3.42 & $ -0.40$ & \nodata & \nodata & \nodata & \nodata &    32.3 &    4.72 & \nodata & \nodata &    59.9 &    5.44 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4174.91 &  0.91 & $ -2.94$ &    77.1 &    4.68 &    51.4 &    4.60 &    56.1 &    4.81 & \nodata & \nodata &    61.7 &    5.24 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4175.64 &  2.85 & $ -0.83$ &    58.9 &    4.65 &    38.5 &    4.53 & \nodata & \nodata & \nodata & \nodata &    51.3 &    5.08 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4181.76 &  2.83 & $ -0.37$ &    72.9 &    4.40 &    47.7 &    4.20 &    46.7 &    4.29 &    31.8 &    4.02 &    74.0 &    5.09 & \nodata & \nodata & \nodata & \nodata &    70.8 &    5.30 & \nodata & \nodata \\
Fe I  &  4184.89 &  2.83 & $ -0.87$ &    37.4 &    4.31 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    76.0 &    5.64 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4187.04 &  2.45 & $ -0.51$ &    80.2 &    4.20 &    87.2 &    4.62 &    73.4 &    4.49 &    49.3 &    4.06 &    90.2 &    5.14 &    80.2 &    5.05 & \nodata & \nodata &    82.0 &    5.23 & \nodata & \nodata \\
Fe I  &  4187.80 &  2.42 & $ -0.51$ &    95.3 &    4.47 &    63.4 &    4.13 &    72.1 &    4.44 &    63.8 &    4.31 &    87.2 &    5.04 &    53.7 &    4.41 & \nodata & \nodata &    96.5 &    5.50 & \nodata & \nodata \\
Fe I  &  4191.43 &  2.47 & $ -0.67$ &    87.2 &    4.52 &    58.8 &    4.27 &    55.9 &    4.34 &    59.6 &    4.44 &    73.5 &    4.94 &    59.5 &    4.74 & \nodata & \nodata &    89.2 &    5.57 & \nodata & \nodata \\
Fe I  &  4195.33 &  3.33 & $ -0.49$ &    45.0 &    4.66 & \nodata & \nodata &    23.5 &    4.51 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4196.21 &  3.40 & $ -0.70$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    44.3 &    5.40 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4199.10 &  3.05 & $  0.16$ &    83.8 &    4.33 &    80.3 &    4.52 &    60.9 &    4.27 &    37.2 &    3.85 &    78.6 &    4.91 &    67.8 &    4.78 & \nodata & \nodata & \nodata & \nodata &    49.7 &    4.58 \\
Fe I  &  4202.03 &  1.49 & $ -0.69$ &   129.4 &    4.26 &   114.0 &    4.32 &   116.7 &    4.63 &    95.9 &    4.22 &   120.8 &    5.03 &    91.7 &    4.55 &    63.3 &    3.86 &   108.9 &    5.12 &    83.2 &    4.64 \\
Fe I  &  4216.18 &  0.00 & $ -3.36$ &   102.7 &    4.45 &    91.4 &    4.67 &    86.9 &    4.81 &    64.3 &    4.37 &    86.7 &    5.21 &    69.5 &    4.96 & \nodata & \nodata &    77.3 &    5.42 & \nodata & \nodata \\
Fe I  &  4222.21 &  2.45 & $ -0.91$ &    58.5 &    4.23 & \nodata & \nodata &    42.0 &    4.30 &    37.0 &    4.23 &    75.8 &    5.21 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4227.43 &  3.33 & $  0.27$ &    74.2 &    4.38 &    78.5 &    4.69 & \nodata & \nodata &    53.9 &    4.37 &    90.3 &    5.37 &    69.5 &    5.00 & \nodata & \nodata &    86.6 &    5.54 & \nodata & \nodata \\
Fe I  &  4233.60 &  2.48 & $ -0.58$ &    75.2 &    4.22 &    69.0 &    4.36 &    66.4 &    4.45 &    43.9 &    4.06 &    88.6 &    5.20 &    66.6 &    4.82 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4238.81 &  3.40 & $ -0.23$ &    43.9 &    4.46 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    62.7 &    5.29 & \nodata & \nodata & \nodata & \nodata &    50.9 &    5.26 & \nodata & \nodata \\
Fe I  &  4247.43 &  3.37 & $ -0.24$ & \nodata & \nodata & \nodata & \nodata &    52.4 &    4.86 & \nodata & \nodata &    75.4 &    5.54 &    45.5 &    4.99 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4250.12 &  2.47 & $ -0.38$ &    95.5 &    4.38 &    72.8 &    4.22 &    69.3 &    4.29 &    47.9 &    3.92 &    92.4 &    5.07 &    80.8 &    4.94 & \nodata & \nodata &    83.4 &    5.14 & \nodata & \nodata \\
Fe I  &  4250.79 &  1.56 & $ -0.71$ &   127.7 &    4.31 &   108.8 &    4.28 &   116.2 &    4.71 &    82.2 &    3.95 &   115.7 &    5.01 &    89.3 &    4.57 &    58.0 &    3.83 &   110.0 &    5.22 &    67.9 &    4.32 \\
Fe I  &  4260.47 &  2.40 & $  0.08$ &   109.9 &    4.14 &   102.4 &    4.29 &    94.6 &    4.31 &    79.0 &    4.02 &   116.4 &    5.02 &    93.8 &    4.70 &    64.7 &    4.05 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4271.15 &  2.45 & $ -0.34$ &   100.3 &    4.41 &    81.6 &    4.32 &    79.3 &    4.44 &    62.3 &    4.13 &   120.8 &    5.57 &    89.1 &    5.07 &    33.7 &    3.93 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4271.76 &  1.49 & $ -0.17$ & \nodata & \nodata &   126.8 &    4.07 &   125.9 &    4.30 &   111.1 &    4.06 & \nodata & \nodata &   122.2 &    4.69 &    88.0 &    3.92 & \nodata & \nodata &   129.4 &    4.95 \\
Fe I  &  4282.40 &  2.18 & $ -0.78$ &    99.7 &    4.52 &    77.1 &    4.37 &    89.2 &    4.83 &    47.7 &    3.99 &   100.7 &    5.45 &    55.7 &    4.47 &    43.1 &    4.28 & \nodata & \nodata &    52.6 &    4.67 \\
Fe I  &  4325.76 &  1.61 & $  0.01$ & \nodata & \nodata & \nodata & \nodata &   135.0 &    4.41 &   118.3 &    4.17 & \nodata & \nodata &   124.9 &    4.67 &    89.2 &    3.89 & \nodata & \nodata &   115.2 &    4.68 \\
Fe I  &  4337.05 &  1.56 & $ -1.70$ &    96.3 &    4.59 &    83.8 &    4.68 &    54.3 &    4.28 &    55.6 &    4.34 &    99.8 &    5.61 &    66.5 &    4.94 & \nodata & \nodata &    89.2 &    5.72 & \nodata & \nodata \\
Fe I  &  4352.73 &  2.22 & $ -1.29$ &    79.5 &    4.66 &    62.0 &    4.64 &    43.5 &    4.44 & \nodata & \nodata &    87.5 &    5.64 & \nodata & \nodata & \nodata & \nodata &    56.7 &    5.21 & \nodata & \nodata \\
Fe I  &  4375.93 &  0.00 & $ -3.00$ &   124.6 &    4.51 &   107.9 &    4.65 &   102.8 &    4.80 &    61.8 &    3.93 &   102.3 &    5.21 &    85.9 &    5.02 &    41.6 &    4.09 &    98.9 &    5.60 & \nodata & \nodata \\
Fe I  &  4383.55 &  1.48 & $  0.20$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   131.4 &    4.08 & \nodata & \nodata &   135.3 &    4.48 &   112.7 &    4.06 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4404.75 &  1.56 & $ -0.15$ & \nodata & \nodata & \nodata & \nodata &   127.9 &    4.35 &   114.3 &    4.16 & \nodata & \nodata &   121.2 &    4.69 &    92.2 &    4.05 & \nodata & \nodata &   108.6 &    4.67 \\
Fe I  &  4407.71 &  2.18 & $ -1.97$ &    39.8 &    4.65 &    35.3 &    4.81 & \nodata & \nodata & \nodata & \nodata &    49.2 &    5.41 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4415.12 &  1.61 & $ -0.62$ &   132.9 &    4.33 &   118.2 &    4.42 &   101.4 &    4.26 &    89.7 &    4.07 &   127.5 &    5.16 &   102.7 &    4.84 &    56.3 &    3.74 &   113.1 &    5.20 &    86.8 &    4.74 \\
Fe I  &  4422.57 &  2.85 & $ -1.11$ &    42.4 &    4.64 &    38.8 &    4.79 & \nodata & \nodata & \nodata & \nodata &    41.9 &    5.15 & \nodata & \nodata & \nodata & \nodata &    40.1 &    5.33 & \nodata & \nodata \\
Fe I  &  4427.31 &  0.05 & $ -2.92$ &   135.5 &    4.71 &   102.3 &    4.48 &    87.7 &    4.39 &    84.7 &    4.42 &   121.2 &    5.64 &    87.5 &    5.04 &    34.1 &    3.91 &    88.0 &    5.29 & \nodata & \nodata \\
Fe I  &  4430.61 &  2.22 & $ -1.66$ &    37.8 &    4.35 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    51.2 &    5.44 & \nodata & \nodata \\
Fe I  &  4442.34 &  2.20 & $ -1.23$ &    84.1 &    4.65 &    55.8 &    4.44 &    53.9 &    4.52 &    28.4 &    4.06 &    84.4 &    5.44 &    43.7 &    4.66 & \nodata & \nodata &    62.1 &    5.23 & \nodata & \nodata \\
Fe I  &  4443.19 &  2.86 & $ -1.04$ & \nodata & \nodata & \nodata & \nodata &    39.3 &    4.83 & \nodata & \nodata &    41.3 &    5.08 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4447.72 &  2.22 & $ -1.34$ &    65.2 &    4.46 &    50.8 &    4.49 &    43.6 &    4.48 &    31.0 &    4.26 &    74.6 &    5.34 & \nodata & \nodata & \nodata & \nodata &    75.2 &    5.67 & \nodata & \nodata \\
Fe I  &  4454.38 &  2.83 & $ -1.30$ & \nodata & \nodata & \nodata & \nodata &    21.0 &    4.67 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4459.12 &  2.18 & $ -1.28$ &    77.5 &    4.55 &    58.4 &    4.51 &    47.0 &    4.43 &    30.4 &    4.14 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4461.65 &  0.09 & $ -3.19$ &   106.5 &    4.40 &   100.1 &    4.74 &    87.7 &    4.71 &    64.7 &    4.27 &   102.9 &    5.49 &    74.6 &    4.98 & \nodata & \nodata &    89.9 &    5.63 &    48.8 &    4.74 \\
Fe I  &  4466.55 &  2.83 & $ -0.60$ &    76.8 &    4.65 &    56.5 &    4.55 &    61.6 &    4.76 &    30.4 &    4.20 &    72.3 &    5.23 &    37.2 &    4.59 & \nodata & \nodata &    61.3 &    5.27 & \nodata & \nodata \\
Fe I  &  4476.02 &  2.85 & $ -0.82$ &    41.3 &    4.33 &    36.4 &    4.46 & \nodata & \nodata &    19.0 &    4.17 &    59.1 &    5.19 & \nodata & \nodata & \nodata & \nodata &    44.9 &    5.14 & \nodata & \nodata \\
Fe I  &  4489.74 &  0.12 & $ -3.90$ &    77.2 &    4.60 &    44.5 &    4.47 &    50.7 &    4.71 &    28.7 &    4.33 &    56.7 &    5.16 & \nodata & \nodata & \nodata & \nodata &    53.9 &    5.47 & \nodata & \nodata \\
Fe I  &  4494.56 &  2.20 & $ -1.14$ &    69.0 &    4.29 &    56.6 &    4.36 &    62.2 &    4.58 &    31.1 &    4.03 &    75.2 &    5.13 & \nodata & \nodata & \nodata & \nodata &    60.8 &    5.10 & \nodata & \nodata \\
Fe I  &  4528.61 &  2.18 & $ -0.82$ &    92.7 &    4.36 &    95.5 &    4.74 &    87.6 &    4.76 &    51.0 &    4.06 &   110.6 &    5.60 &    66.7 &    4.72 & \nodata & \nodata &    87.6 &    5.40 &    55.5 &    4.73 \\
Fe I  &  4531.15 &  1.48 & $ -2.10$ &    82.1 &    4.58 &    52.5 &    4.40 &    53.4 &    4.54 & \nodata & \nodata &    84.3 &    5.50 & \nodata & \nodata & \nodata & \nodata &    62.3 &    5.33 & \nodata & \nodata \\
Fe I  &  4592.65 &  1.56 & $ -2.46$ &    57.4 &    4.64 & \nodata & \nodata &    35.9 &    4.68 &    18.1 &    4.30 &    73.2 &    5.68 & \nodata & \nodata & \nodata & \nodata &    51.5 &    5.53 & \nodata & \nodata \\
Fe I  &  4602.94 &  1.49 & $ -2.21$ &    86.7 &    4.77 &    49.1 &    4.46 &    60.3 &    4.78 &    25.0 &    4.14 &    70.9 &    5.30 & \nodata & \nodata & \nodata & \nodata &    70.5 &    5.65 & \nodata & \nodata \\
Fe I  &  4632.91 &  1.61 & $ -2.91$ & \nodata & \nodata &    26.2 &    4.89 & \nodata & \nodata & \nodata & \nodata &    33.6 &    5.40 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4647.43 &  2.95 & $ -1.35$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    39.6 &    5.44 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4691.41 &  2.99 & $ -1.52$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    33.2 &    5.53 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4707.27 &  3.24 & $ -1.08$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    40.3 &    5.49 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4733.59 &  1.49 & $ -2.99$ &    24.5 &    4.51 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4736.77 &  3.21 & $ -0.75$ &    26.5 &    4.40 &    18.9 &    4.40 &    20.2 &    4.51 & \nodata & \nodata &    52.5 &    5.36 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4859.74 &  2.88 & $ -0.76$ &    53.8 &    4.47 &    63.3 &    4.84 & \nodata & \nodata &    19.4 &    4.13 &    74.5 &    5.43 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4871.32 &  2.87 & $ -0.36$ &    76.5 &    4.41 &    74.0 &    4.61 &    69.4 &    4.66 &    38.4 &    4.13 &    74.0 &    5.01 & \nodata & \nodata & \nodata & \nodata &    83.9 &    5.46 & \nodata & \nodata \\
Fe I  &  4872.14 &  2.88 & $ -0.57$ &    48.2 &    4.20 &    70.8 &    4.78 &    60.7 &    4.72 &    26.3 &    4.11 &    67.1 &    5.09 & \nodata & \nodata & \nodata & \nodata &    88.5 &    5.78 &    46.2 &    4.97 \\
Fe I  &  4890.76 &  2.88 & $ -0.39$ &    82.7 &    4.55 &    79.9 &    4.75 &    59.5 &    4.52 &    38.6 &    4.18 &    77.7 &    5.12 & \nodata & \nodata & \nodata & \nodata &    78.9 &    5.40 &    48.9 &    4.84 \\
Fe I  &  4891.49 &  2.85 & $ -0.11$ &    79.7 &    4.18 &    67.6 &    4.23 &    63.4 &    4.27 &    49.0 &    4.05 &    96.7 &    5.21 & \nodata & \nodata & \nodata & \nodata &    78.9 &    5.09 &    51.3 &    4.58 \\
Fe I  &  4903.31 &  2.88 & $ -0.93$ &    37.9 &    4.39 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    70.5 &    5.51 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4918.99 &  2.85 & $ -0.34$ &    72.8 &    4.29 & \nodata & \nodata &    66.7 &    4.56 &    38.6 &    4.09 &    89.1 &    5.28 & \nodata & \nodata & \nodata & \nodata &    87.0 &    5.48 & \nodata & \nodata \\
Fe I  &  4920.50 &  2.83 & $  0.07$ &   112.2 &    4.56 & \nodata & \nodata &    90.5 &    4.60 & \nodata & \nodata &   127.0 &    5.55 &    76.7 &    4.70 & \nodata & \nodata &   115.6 &    5.55 & \nodata & \nodata \\
Fe I  &  4938.81 &  2.88 & $ -1.08$ &    30.2 &    4.39 &    39.2 &    4.77 & \nodata & \nodata & \nodata & \nodata &    50.1 &    5.27 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4939.69 &  0.86 & $ -3.25$ &    56.8 &    4.51 &    33.8 &    4.47 & \nodata & \nodata &    24.0 &    4.40 &    75.8 &    5.69 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4994.13 &  0.92 & $ -2.97$ &    56.8 &    4.30 &    40.8 &    4.38 &    58.9 &    4.81 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5001.87 &  3.88 & $  0.05$ & \nodata & \nodata &    28.9 &    4.59 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5012.07 &  0.86 & $ -2.64$ &    84.8 &    4.31 & \nodata & \nodata &    68.2 &    4.56 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5041.07 &  0.96 & $ -3.09$ &    62.0 &    4.54 & \nodata & \nodata &    53.5 &    4.88 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5041.76 &  1.49 & $ -2.20$ &    85.6 &    4.66 & \nodata & \nodata &    48.2 &    4.52 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5049.82 &  2.28 & $ -1.35$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    33.6 &    4.34 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5051.63 &  0.92 & $ -2.76$ &    96.4 &    4.70 &    77.9 &    4.76 &    59.5 &    4.60 & \nodata & \nodata &    78.0 &    5.31 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5068.77 &  2.94 & $ -1.04$ &    37.1 &    4.54 &    38.8 &    4.78 & \nodata & \nodata & \nodata & \nodata &    61.6 &    5.50 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5079.74 &  0.99 & $ -3.25$ &    50.7 &    4.57 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5083.34 &  0.96 & $ -2.84$ &    76.8 &    4.50 &    35.4 &    4.20 &    44.7 &    4.48 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5110.41 &  0.00 & $ -3.76$ &    99.0 &    4.57 &    80.4 &    4.70 &    60.0 &    4.51 &    37.3 &    4.17 &    95.0 &    5.64 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5123.72 &  1.01 & $ -3.06$ &    81.3 &    4.85 &    50.3 &    4.72 &    50.4 &    4.84 & \nodata & \nodata &    77.9 &    5.70 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5127.36 &  0.92 & $ -3.25$ &    56.6 &    4.57 &    38.4 &    4.61 & \nodata & \nodata & \nodata & \nodata &    57.2 &    5.37 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5142.93 &  0.96 & $ -3.08$ &    80.3 &    4.79 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    64.5 &    5.38 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5150.84 &  0.99 & $ -3.04$ &    57.5 &    4.46 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5151.91 &  1.01 & $ -3.32$ &    39.8 &    4.50 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    54.0 &    5.48 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5166.28 &  0.00 & $ -4.12$ &    88.4 &    4.74 &    68.4 &    4.85 &    56.3 &    4.81 & \nodata & \nodata &    62.0 &    5.28 & \nodata & \nodata & \nodata & \nodata &    55.0 &    5.51 & \nodata & \nodata \\
Fe I  &  5171.60 &  1.49 & $ -1.72$ &    96.1 &    4.35 &    73.5 &    4.31 &    67.1 &    4.35 &    65.1 &    4.37 &   106.9 &    5.56 & \nodata & \nodata & \nodata & \nodata &    80.0 &    5.31 & \nodata & \nodata \\
Fe I  &  5191.45 &  3.04 & $ -0.55$ &    74.6 &    4.74 &    51.7 &    4.61 &    37.5 &    4.46 & \nodata & \nodata &    62.5 &    5.13 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5192.34 &  3.00 & $ -0.42$ &    56.8 &    4.29 &    38.4 &    4.22 & \nodata & \nodata &    26.2 &    4.07 &    69.7 &    5.10 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5194.94 &  1.56 & $ -2.02$ &    74.8 &    4.39 & \nodata & \nodata & \nodata & \nodata &    40.1 &    4.29 &    80.4 &    5.33 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5216.27 &  1.61 & $ -2.08$ &    70.8 &    4.45 &    56.2 &    4.53 & \nodata & \nodata & \nodata & \nodata &    70.3 &    5.23 & \nodata & \nodata & \nodata & \nodata &    63.6 &    5.41 & \nodata & \nodata \\
Fe I  &  5225.53 &  0.11 & $ -4.75$ &    31.4 &    4.66 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5232.94 &  2.94 & $ -0.06$ &    78.8 &    4.19 &    64.2 &    4.20 &    62.9 &    4.29 & \nodata & \nodata &   104.3 &    5.37 & \nodata & \nodata & \nodata & \nodata &    86.2 &    5.26 &    40.0 &    4.38 \\
Fe I  &  5250.21 &  0.12 & $ -4.94$ &    26.8 &    4.77 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5250.65 &  2.20 & $ -2.18$ &    28.1 &    4.61 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5254.96 &  0.11 & $ -4.76$ &    32.5 &    4.69 &    21.4 &    4.81 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5266.56 &  3.00 & $ -0.39$ &    53.9 &    4.22 &    44.5 &    4.28 &    61.0 &    4.66 &    30.3 &    4.13 &    81.4 &    5.30 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5269.54 &  0.86 & $ -1.33$ & \nodata & \nodata &   148.8 &    4.66 &   142.1 &    4.78 &   101.0 &    4.03 &   137.0 &    5.04 &   105.4 &    4.64 &    67.6 &    3.79 &   126.6 &    5.22 &   102.3 &    4.89 \\
Fe I  &  5281.79 &  3.04 & $ -0.83$ &    53.0 &    4.69 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5283.62 &  3.24 & $ -0.52$ &    37.4 &    4.38 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    54.2 &    5.17 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5302.30 &  3.28 & $ -0.72$ & \nodata & \nodata &    28.3 &    4.65 &    29.3 &    4.74 & \nodata & \nodata &    58.7 &    5.49 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5307.36 &  1.61 & $ -2.91$ &    31.6 &    4.68 & \nodata & \nodata &    25.1 &    4.91 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5324.18 &  3.21 & $ -0.10$ &    62.0 &    4.30 & \nodata & \nodata &    50.3 &    4.42 &    34.6 &    4.16 &    95.6 &    5.52 &    45.3 &    4.61 & \nodata & \nodata &    77.3 &    5.39 & \nodata & \nodata \\
Fe I  &  5328.04 &  0.92 & $ -1.47$ &   162.8 &    4.58 &   141.9 &    4.73 &   124.8 &    4.64 &   101.8 &    4.25 &   149.2 &    5.42 &   119.1 &    5.12 &    64.6 &    3.93 &   117.0 &    5.25 &    86.0 &    4.72 \\
Fe I  &  5328.53 &  1.56 & $ -1.85$ &    87.3 &    4.40 &    66.7 &    4.40 &    70.1 &    4.60 &    47.2 &    4.24 &    84.0 &    5.23 & \nodata & \nodata & \nodata & \nodata &    95.8 &    5.87 & \nodata & \nodata \\
Fe I  &  5339.93 &  3.27 & $ -0.72$ &    32.1 &    4.52 & \nodata & \nodata &    30.6 &    4.75 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5369.96 &  4.37 & $  0.54$ & \nodata & \nodata &    25.6 &    4.58 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5371.49 &  0.96 & $ -1.64$ &   142.4 &    4.42 &   117.0 &    4.42 &   115.5 &    4.64 &   101.3 &    4.45 &   116.7 &    5.06 &   104.9 &    5.03 &    72.8 &    4.32 &   111.2 &    5.34 &    80.1 &    4.79 \\
Fe I  &  5383.37 &  4.31 & $  0.65$ & \nodata & \nodata &    20.3 &    4.27 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5393.17 &  3.24 & $ -0.91$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    33.9 &    5.17 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5397.13 &  0.92 & $ -1.98$ &   134.1 &    4.55 &   122.2 &    4.82 &   118.0 &    4.99 &    79.8 &    4.24 &   103.9 &    5.07 &   100.9 &    5.23 & \nodata & \nodata &   101.2 &    5.43 &    84.7 &    5.19 \\
Fe I  &  5405.77 &  0.99 & $ -1.85$ &   127.7 &    4.39 &   130.3 &    4.94 &   101.1 &    4.56 &    73.7 &    4.06 &   131.2 &    5.58 &    96.2 &    5.07 &    51.4 &    4.12 & \nodata & \nodata &    59.8 &    4.53 \\
Fe I  &  5415.20 &  4.39 & $  0.64$ & \nodata & \nodata &    24.7 &    4.48 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5429.70 &  0.96 & $ -1.88$ &   146.4 &    4.72 &   126.4 &    4.85 &   105.1 &    4.64 &    85.6 &    4.31 &   118.7 &    5.33 &    77.2 &    4.59 & \nodata & \nodata &   115.2 &    5.65 & \nodata & \nodata \\
Fe I  &  5434.52 &  1.01 & $ -2.13$ &   127.2 &    4.68 &   101.5 &    4.64 &    97.0 &    4.77 &    74.6 &    4.38 &   106.9 &    5.39 &    67.9 &    4.67 & \nodata & \nodata &   105.4 &    5.76 &    68.8 &    5.04 \\
Fe I  &  5446.92 &  0.99 & $ -1.91$ &   135.0 &    4.57 &    92.9 &    4.23 &   116.9 &    4.97 &    73.3 &    4.11 &   121.5 &    5.45 &    70.5 &    4.49 & \nodata & \nodata &   104.4 &    5.49 &    71.5 &    4.87 \\
Fe I  &  5455.61 &  1.01 & $ -2.09$ &   124.8 &    4.59 &    88.4 &    4.34 &   102.3 &    4.84 &    82.4 &    4.51 &   105.4 &    5.31 &    68.2 &    4.64 & \nodata & \nodata & \nodata & \nodata &    60.8 &    4.81 \\
Fe I  &  5497.52 &  1.01 & $ -2.83$ &    87.0 &    4.66 &    74.6 &    4.84 &    53.5 &    4.64 & \nodata & \nodata &    64.4 &    5.16 &    58.3 &    5.16 & \nodata & \nodata &    70.0 &    5.63 & \nodata & \nodata \\
Fe I  &  5501.47 &  0.96 & $ -3.05$ &    71.0 &    4.58 &    39.1 &    4.44 & \nodata & \nodata &    17.8 &    4.12 &    72.9 &    5.49 & \nodata & \nodata & \nodata & \nodata &    65.4 &    5.70 & \nodata & \nodata \\
Fe I  &  5506.78 &  0.99 & $ -2.79$ &    84.7 &    4.56 &    62.6 &    4.59 &    56.8 &    4.63 &    29.3 &    4.17 &    72.0 &    5.25 &    45.3 &    4.83 & \nodata & \nodata &    69.0 &    5.55 & \nodata & \nodata \\
Fe I  &  5569.62 &  3.42 & $ -0.54$ & \nodata & \nodata &    14.7 &    4.26 & \nodata & \nodata & \nodata & \nodata &    41.9 &    5.15 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5572.84 &  3.40 & $ -0.28$ &    36.0 &    4.29 &    33.1 &    4.43 &    37.6 &    4.58 & \nodata & \nodata &    52.0 &    5.05 & \nodata & \nodata & \nodata & \nodata &    64.9 &    5.50 & \nodata & \nodata \\
Fe I  &  5586.76 &  3.37 & $ -0.14$ &    47.0 &    4.29 &    64.2 &    4.76 &    48.5 &    4.60 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5615.64 &  3.33 & $  0.05$ &    73.1 &    4.43 & \nodata & \nodata &    43.5 &    4.28 & \nodata & \nodata &    75.9 &    5.09 &    44.8 &    4.57 & \nodata & \nodata &    68.7 &    5.17 & \nodata & \nodata \\
Fe I  &  5624.54 &  3.42 & $ -0.76$ &    24.6 &    4.57 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5658.82 &  3.40 & $ -0.79$ & \nodata & \nodata &    23.4 &    4.73 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6065.48 &  2.61 & $ -1.41$ &    35.1 &    4.41 & \nodata & \nodata &    27.4 &    4.58 & \nodata & \nodata &    59.0 &    5.42 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6136.61 &  2.45 & $ -1.41$ &    50.8 &    4.46 &    38.1 &    4.51 &    50.0 &    4.80 & \nodata & \nodata &    67.8 &    5.40 & \nodata & \nodata & \nodata & \nodata &    66.0 &    5.65 & \nodata & \nodata \\
Fe I  &  6137.69 &  2.59 & $ -1.35$ &    39.6 &    4.40 &    53.5 &    4.86 & \nodata & \nodata & \nodata & \nodata &    73.6 &    5.62 & \nodata & \nodata & \nodata & \nodata &    51.2 &    5.43 & \nodata & \nodata \\
Fe I  &  6191.56 &  2.43 & $ -1.42$ &    60.4 &    4.58 &    32.2 &    4.39 & \nodata & \nodata & \nodata & \nodata &    84.4 &    5.73 & \nodata & \nodata & \nodata & \nodata &    64.4 &    5.60 & \nodata & \nodata \\
Fe I  &  6230.72 &  2.56 & $ -1.28$ &    43.7 &    4.35 &    44.4 &    4.61 & \nodata & \nodata & \nodata & \nodata &    57.8 &    5.20 & \nodata & \nodata & \nodata & \nodata &    50.8 &    5.31 & \nodata & \nodata \\
Fe I  &  6252.56 &  2.40 & $ -1.69$ &    48.4 &    4.63 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    49.9 &    5.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6265.13 &  2.18 & $ -2.54$ & \nodata & \nodata &    19.5 &    4.93 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6335.33 &  2.20 & $ -2.18$ &    31.6 &    4.60 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6393.60 &  2.43 & $ -1.58$ &    57.0 &    4.68 &    21.4 &    4.30 &    33.4 &    4.65 & \nodata & \nodata &    57.5 &    5.34 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6400.00 &  3.60 & $ -0.29$ & \nodata & \nodata &    31.9 &    4.61 & \nodata & \nodata & \nodata & \nodata &    44.3 &    5.11 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6421.35 &  2.28 & $ -2.01$ &    27.1 &    4.44 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    53.6 &    5.53 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6430.85 &  2.18 & $ -1.95$ &    43.5 &    4.54 &    27.8 &    4.52 & \nodata & \nodata & \nodata & \nodata &    49.2 &    5.28 & \nodata & \nodata & \nodata & \nodata &    37.8 &    5.31 & \nodata & \nodata \\
Fe I  &  6494.98 &  2.40 & $ -1.24$ &    67.7 &    4.44 &    35.0 &    4.20 &    43.0 &    4.44 &    20.9 &    4.01 &    78.0 &    5.36 & \nodata & \nodata & \nodata & \nodata &    79.3 &    5.69 & \nodata & \nodata \\
Fe I  &  6592.91 &  2.73 & $ -1.47$ &    27.8 &    4.46 &    26.8 &    4.66 & \nodata & \nodata & \nodata & \nodata &    31.8 &    5.08 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6677.99 &  2.69 & $ -1.42$ &    43.2 &    4.62 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4178.86 &  2.58 & $ -2.51$ & \nodata & \nodata & \nodata & \nodata &    35.2 &    4.51 & \nodata & \nodata &    52.9 &    5.18 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4233.17 &  2.58 & $ -1.97$ &    80.9 &    4.43 &    73.0 &    4.53 &    61.6 &    4.45 & \nodata & \nodata &    89.6 &    5.47 & \nodata & \nodata & \nodata & \nodata &    76.7 &    5.48 & \nodata & \nodata \\
Fe II &  4416.82 &  2.78 & $ -2.60$ & \nodata & \nodata &    36.6 &    4.74 &    36.8 &    4.83 & \nodata & \nodata &    38.4 &    5.19 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4491.41 &  2.86 & $ -2.71$ & \nodata & \nodata & \nodata & \nodata &    19.1 &    4.64 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4508.28 &  2.86 & $ -2.58$ & \nodata & \nodata &    34.4 &    4.77 & \nodata & \nodata & \nodata & \nodata &    43.0 &    5.34 & \nodata & \nodata & \nodata & \nodata &    43.7 &    5.58 & \nodata & \nodata \\
Fe II &  4515.34 &  2.84 & $ -2.60$ & \nodata & \nodata & \nodata & \nodata &    26.3 &    4.68 & \nodata & \nodata &    48.9 &    5.45 & \nodata & \nodata & \nodata & \nodata &    35.6 &    5.41 & \nodata & \nodata \\
Fe II &  4520.22 &  2.81 & $ -2.60$ &    35.6 &    4.55 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    39.8 &    5.24 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4522.63 &  2.84 & $ -2.25$ & \nodata & \nodata & \nodata & \nodata &    46.6 &    4.72 & \nodata & \nodata &    66.1 &    5.44 & \nodata & \nodata & \nodata & \nodata &    54.8 &    5.46 & \nodata & \nodata \\
Fe II &  4555.89 &  2.83 & $ -2.40$ & \nodata & \nodata &    45.5 &    4.75 & \nodata & \nodata & \nodata & \nodata &    45.8 &    5.18 & \nodata & \nodata & \nodata & \nodata &    43.9 &    5.37 & \nodata & \nodata \\
Fe II &  4583.84 &  2.81 & $ -1.93$ &    69.0 &    4.41 &    56.0 &    4.42 &    57.5 &    4.56 &    40.8 &    4.34 &    80.4 &    5.40 &    45.0 &    4.69 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4923.93 &  2.89 & $ -1.32$ &    96.9 &    4.33 &    87.2 &    4.42 &    81.3 &    4.46 &    53.3 &    4.02 &   104.0 &    5.40 &    68.2 &    4.65 & \nodata & \nodata &    92.3 &    5.45 & \nodata & \nodata \\
Fe II &  5018.45 &  2.89 & $ -1.22$ &   108.6 &    4.43 & \nodata & \nodata &    84.6 &    4.42 &    63.5 &    4.10 &   105.7 &    5.32 &    84.6 &    4.94 & \nodata & \nodata &    91.1 &    5.30 & \nodata & \nodata \\
Fe II &  5197.58 &  3.23 & $ -2.22$ & \nodata & \nodata &    31.3 &    4.74 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  5276.00 &  3.20 & $ -2.01$ & \nodata & \nodata &    45.6 &    4.74 &    37.7 &    4.69 & \nodata & \nodata &    51.6 &    5.27 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co I  &  3845.47 &  0.92 & $  0.01$ & \nodata & \nodata & \nodata & \nodata &    80.1 &    2.33 & \nodata & \nodata &    87.0 &    2.87 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co I  &  3873.12 &  0.43 & $ -0.66$ &    88.5 &    1.97 & \nodata & \nodata &    81.3 &    2.45 & \nodata & \nodata &    93.1 &    3.15 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co I  &  3881.87 &  0.58 & $ -1.13$ & \nodata & \nodata & \nodata & \nodata &    61.8 &    2.63 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co I  &  3995.31 &  0.92 & $ -0.22$ &    62.3 &    1.62 &    74.5 &    2.18 &    83.2 &    2.59 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co I  &  4020.90 &  0.43 & $ -2.07$ &    36.5 &    2.43 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co I  &  4110.53 &  1.05 & $ -1.08$ &    35.4 &    2.18 &    45.0 &    2.66 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co I  &  4118.77 &  1.05 & $ -0.49$ &    55.9 &    1.92 &    69.0 &    2.47 &    49.2 &    2.27 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co I  &  4121.32 &  0.92 & $ -0.32$ &    86.3 &    2.12 &    63.2 &    2.05 & \nodata & \nodata &    69.0 &    2.39 & \nodata & \nodata & $< 93.3$& $< 3.51$& $< 84.4$& $< 2.60$& $<117.7$& $< 4.24$& $< 93.2$& $< 3.84$\\
Ni I  &  3783.52 &  0.42 & $ -1.42$ &   105.3 &    3.00 &    91.4 &    3.08 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ni I  &  3807.14 &  0.42 & $ -1.22$ &   104.5 &    2.77 &    92.9 &    2.92 & \nodata & \nodata &    63.2 &    2.58 &    99.3 &    3.74 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ni I  &  3858.30 &  0.42 & $ -0.95$ &   128.7 &    3.05 & \nodata & \nodata &   103.5 &    3.18 &    68.8 &    2.84 & \nodata & \nodata & $<192.1$& $< 4.86$& $<186.4$& $< 4.76$& $<131.9$& $< 4.46$& $<202.1$& $< 5.01$\\
Ni I  &  5476.90 &  1.83 & $ -0.89$ &    80.2 &    3.36 &    56.4 &    3.30 &    57.7 &    3.44 & \nodata & \nodata &    91.7 &    4.46 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Zn I  &  4722.15 &  4.03 & $ -0.39$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    60.1 &    3.44 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Zn I  &  4810.53 &  4.08 & $ -0.14$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    55.0 &    3.13 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sr II &  4077.71 &  0.00 & $  0.15$ &     syn &    0.06 &     syn &    0.55 &     syn &    0.37 &     syn & $<-1.37$&     syn &    0.38 &     syn &    0.54 &     syn & $<-0.67$&     syn &    1.09 & \nodata & \nodata \\
Sr II &  4215.52 &  0.00 & $ -0.18$ &     syn &    0.01 &     syn &    0.50 &     syn &    0.26 &     syn & $<-1.37$&     syn &    0.28 &     syn &    0.19 &     syn & $<-0.67$&     syn &    1.24 &     syn &    0.40 \\
Y II  &  3774.33 &  0.13 & $  0.21$ &    95.0 &   -0.80 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Y II  &  3788.69 &  0.10 & $ -0.07$ &   108.3 &   -0.25 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Y II  &  3818.34 &  0.13 & $ -0.98$ &    72.3 &   -0.10 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Y II  &  3950.35 &  0.10 & $ -0.49$ &    72.5 &   -0.66 &    79.1 &   -0.12 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    62.5 &    0.33 & \nodata & \nodata &    77.1 &    1.08 & \nodata & \nodata \\
Y II  &  4398.01 &  0.13 & $ -1.00$ &    66.7 &   -0.29 &    70.6 &    0.15 &    35.6 &   -0.31 & \nodata & \nodata &    27.4 &   -0.03 &    50.1 &    0.48 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Y II  &  4682    &\nodata&  \nodata &     syn &   -0.43 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Y II  &  4854    &\nodata&  \nodata &     syn &   -0.80 &     syn &   -0.20 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Y II  &  4883.68 &  1.08 & $  0.07$ &    51.2 &   -0.46 &    44.8 &   -0.27 &    40.5 &   -0.22 & \nodata & \nodata &    24.6 &   -0.14 & \nodata & \nodata & \nodata & \nodata &    57.7 &    0.88 & \nodata & \nodata \\
Y II  &  4900    &\nodata&  \nodata &     syn &   -0.55 &     syn &   -0.16 &     syn &   -0.10 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Zr II &  3836.76 &  0.56 & $ -0.06$ & \nodata & \nodata &    88.7 &    0.72 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Zr II &  3998.97 &  0.56 & $ -0.52$ &    55.8 &    0.12 &    48.2 &    0.33 &    56.1 &    0.63 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Zr II &  4149.20 &  0.80 & $ -0.03$ &    68.3 &    0.11 &    63.1 &    0.36 &    59.2 &    0.45 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Zr II &  4161.21 &  0.71 & $ -0.72$ & \nodata & \nodata &    37.5 &    0.50 &    45.2 &    0.77 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Zr II &  4208.98 &  0.71 & $ -0.51$ &    40.6 &    0.02 &    41.0 &    0.35 &    43.4 &    0.52 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Zr II &  4496.98 &  0.71 & $ -0.59$ & \nodata & \nodata &    47.8 &    0.51 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ba II &  4554.03 &  0.00 & $  0.16$ &     syn &    0.02 &     syn &    0.21 &     syn &    0.07 &     syn & $<-1.96$&     syn &    0.24 &     syn &    0.95 &     syn & $<-1.26$&     syn &    1.40 &     syn &    0.91 \\
Ba II &  4934.09 &  0.00 & $ -0.16$ &     syn &   -0.03 &     syn &   -0.09 &     syn &    0.77 &     syn & $<-1.96$&     syn &    0.24 &     syn &    1.15 &     syn & $<-0.96$&     syn &    1.50 &     syn &    0.61 \\
Ba II &  5853    &\nodata&  \nodata &     syn &   -0.13 &     syn &    0.31 &     syn &    0.17 & \nodata & \nodata &     syn &    0.29 &     syn &    0.45 & \nodata & \nodata &     syn &    1.40 & \nodata & \nodata \\
Ba II &  6141    &\nodata&  \nodata &     syn &   -0.03 &     syn &   -0.04 &     syn &    0.17 & \nodata & \nodata &     syn &    0.49 &     syn &    0.95 & \nodata & \nodata &     syn &    1.50 &     syn &    0.61 \\
Ba II &  6496.90 &  0.60 & $ -0.37$ &     syn &   -0.03 &     syn &    0.21 &     syn &    0.57 & \nodata & \nodata &     syn &    0.49 &     syn &    0.75 & \nodata & \nodata &     syn &    1.50 &     syn &    1.11 \\
La II &  4077    &\nodata&  \nodata &     syn &   -0.91 &     syn &   -0.67 &     syn &   -0.51 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
La II &  4086    &\nodata&  \nodata & \nodata & \nodata &     syn &   -0.67 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
La II &  4123    &\nodata&  \nodata &     syn &   -0.91 &     syn &   -0.57 &     syn &   -0.51 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
La II &  4429    &\nodata&  \nodata &     syn &   -0.61 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ce II &  4083.22 &  0.70 & $  0.27$ &    27.3 &   -0.46 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ce II &  4137.64 &  0.52 & $  0.40$ &    47.2 &   -0.46 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ce II &  4222.60 &  0.12 & $ -0.15$ &    29.1 &   -0.74 & \nodata & \nodata &    27.5 &   -0.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ce II &  4418.78 &  0.86 & $  0.31$ &    22.4 &   -0.44 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ce II &  4562.36 &  0.48 & $  0.33$ &    43.7 &   -0.54 &    49.5 &   -0.10 &    52.4 &    0.10 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    43.1 &    0.75 & \nodata & \nodata \\
Ce II &  4628.16 &  0.52 & $  0.14$ &    37.2 &   -0.42 &    30.4 &   -0.21 &    40.9 &    0.12 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Pr II &  4062.80 &  0.42 & $  0.33$ & \nodata & \nodata &    35.9 &   -0.48 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Pr II &  4408    &\nodata&  \nodata &     syn &   -1.09 &     syn &   -0.85 &     syn &   -0.79 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Nd II &  3784.25 &  0.38 & $  0.15$ &    56.8 &   -0.39 &    61.3 &    0.07 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Nd II &  3838.98 &  0.00 & $ -0.24$ & \nodata & \nodata &    61.9 &    0.00 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Nd II &  3991.74 &  0.00 & $ -0.26$ &    59.1 &   -0.45 &    50.5 &   -0.21 &    70.1 &    0.38 & \nodata & \nodata &    37.2 &    0.18 & \nodata & \nodata & \nodata & \nodata &    86.0 &    1.93 & \nodata & \nodata \\
Nd II &  4012.70 &  0.00 & $ -0.60$ &    42.9 &   -0.38 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    20.7 &    0.13 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Nd II &  4021.33 &  0.32 & $ -0.17$ &    36.7 &   -0.53 & \nodata & \nodata &    47.1 &    0.18 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Nd II &  4023.00 &  0.56 & $  0.04$ &    28.8 &   -0.59 &    33.8 &   -0.15 &    52.4 &    0.36 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Nd II &  4061.08 &  0.47 & $  0.30$ &    96.8 &    0.29 &    71.0 &    0.16 &    80.3 &    0.62 & \nodata & \nodata &    59.2 &    0.61 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Nd II &  4069.26 &  0.06 & $ -0.40$ &    75.7 &    0.03 &    71.0 &    0.37 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Nd II &  4109.07 &  0.06 & $ -0.16$ &    71.0 &   -0.30 &    56.4 &   -0.15 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Nd II &  4109.45 &  0.32 & $  0.35$ &   101.2 &    0.12 &    59.0 &   -0.31 &    64.4 &   -0.01 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Nd II &  4135.32 &  0.63 & $ -0.07$ &    23.6 &   -0.52 &    25.7 &   -0.14 &    46.8 &    0.42 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Nd II &  4232.37 &  0.06 & $ -0.35$ &    58.7 &   -0.33 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    32.7 &    0.57 & \nodata & \nodata \\
Nd II &  4446.38 &  0.20 & $ -0.63$ &    62.4 &    0.15 &    44.4 &    0.23 &    25.8 &    0.01 & \nodata & \nodata &    26.8 &    0.49 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Nd II &  4462.98 &  0.56 & $ -0.07$ &    69.6 &    0.15 &    41.3 &    0.05 &    34.5 &    0.06 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    42.8 &    1.03 & \nodata & \nodata \\
Nd II &  5319.81 &  0.55 & $ -0.35$ &    36.6 &   -0.19 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sm II &  4318.93 &  0.28 & $ -0.27$ &    43.6 &   -0.64 &    50.8 &   -0.17 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sm II &  4434.32 &  0.38 & $ -0.07$ &    52.8 &   -0.58 & \nodata & \nodata &    44.0 &   -0.23 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sm II &  4467.34 &  0.66 & $  0.15$ &    36.3 &   -0.73 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sm II &  4519.63 &  0.54 & $ -0.35$ & \nodata & \nodata &    21.6 &   -0.36 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sm II &  4537.94 &  0.48 & $ -0.23$ & \nodata & \nodata &    32.8 &   -0.31 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sm II &  4577.69 &  0.25 & $ -0.77$ & \nodata & \nodata & \nodata & \nodata &    34.6 &    0.12 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Eu II &  4129    &\nodata&  \nodata &     syn &   -0.69 &     syn &   -0.90 &     syn &   -0.59 &     syn & $<-1.32$&     syn &   -0.87 &     syn &   -0.51 &     syn & $<-0.62$&     syn &    0.54 &     syn &   -0.14 \\
Eu II &  4205    &\nodata&  \nodata &     syn &   -0.79 &     syn &   -0.85 &     syn &   -0.49 & \nodata & \nodata &     syn &   -0.57 &     syn &   -0.51 & \nodata & \nodata &     syn &    0.14 &     syn &   -0.14 \\
Eu II &  4435    &\nodata&  \nodata &     syn &   -0.79 &     syn &   -0.65 &     syn &   -0.49 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &     syn &   -0.06 & \nodata & \nodata \\
Eu II &  4522    &\nodata&  \nodata &     syn &   -0.99 &     syn &   -0.45 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Eu II &  6645    &\nodata&  \nodata &     syn &   -0.79 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Gd II &  3796.38 &  0.03 & $  0.02$ &    67.1 &   -0.60 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Gd II &  3916.51 &  0.60 & $  0.06$ &    28.9 &   -0.64 &    37.5 &   -0.14 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Gd II &  4191.07 &  0.43 & $ -0.68$ &    26.7 &   -0.18 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Dy II &  3869.86 &  0.00 & $ -0.94$ &    52.6 &   -0.14 & \nodata & \nodata &    55.0 &    0.46 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Dy II &  3944.68 &  0.00 & $  0.11$ &    78.0 &   -0.75 &    99.0 &    0.21 &    76.5 &   -0.09 & \nodata & \nodata &    55.0 &   -0.11 &    44.4 &   -0.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Dy II &  3996.69 &  0.59 & $ -0.19$ & \nodata & \nodata & \nodata & \nodata &    50.0 &    0.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    56.6 &    1.30 & \nodata & \nodata \\
Dy II &  4077    &\nodata&  \nodata &     syn &   -0.41 &     syn &   -0.57 &     syn &    0.29 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Dy II &  4103.31 &  0.10 & $ -0.38$ &    85.1 &   -0.03 &    62.1 &   -0.08 &    59.5 &    0.06 & \nodata & \nodata &    53.7 &    0.42 &    56.2 &    0.60 & \nodata & \nodata &    63.8 &    1.14 & \nodata & \nodata \\
Dy II &  5169.69 &  0.10 & $ -1.66$ &    17.3 &   -0.13 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
\enddata
\end{deluxetable*}

